Rethinking the Setting of Semi-supervised Learning on Graphs

We argue that the present setting of semisupervised learning on graphs may result in unfair comparisons, due to its potential risk of over-tuning hyper-parameters for models. In this paper, we highlight the significant influence of tuning hyper-parameters, which leverages the label information in the validation set to improve the performance. To explore the limit of over-tuning hyperparameters, we propose ValidUtil, an approach to fully utilize the label information in the validation set through an extra group of hyper-parameters. With ValidUtil, even GCN can easily get high accuracy of 85.8% on Cora. To avoid over-tuning, we merge the training set and the validation set and construct an i.i.d. graph benchmark (IGB) consisting of 4 datasets. Each dataset contains 100 i.i.d. graphs sampled from a large graph to reduce the evaluation variance. Our experiments suggest that IGB is a more stable benchmark than previous datasets for semisupervised learning on graphs.

==> related.tex <==

\section{RELATED WORK}

\subsection{GRAPH SAMPLING}
For the graph sampling algorithm, many algorithms have been proposed to make the sampled graphs more valuable and suitable for practical application scenarios. A more detailed survey of the theoretical algorithm is given by Hu and Lau \cite{Hu2013ASA}. Snowball Sampling\cite{biernacki1981snowball} has long been used in sociology studies, where an investigation is performed on a hidden population \cite{biernacki1981snowball}, it can extract some features of the vertices.

There are also a number of random walk-based graph sampling methods called the simple random walk \cite{rasti2009respondent,gjoka2011practical} and Metropolis-Hastings random walk \cite{metropolis1953equation,hastings1970monte,MHRW2009}. The former initiates a simple walk on a graph, moving from a node to one of its randomly chosen neighbors to collect the random sample of nodes; the latter obtains a uniform sample of nodes in a random walk by introducing acceptance probabilities.

\subsection{GRAPH BENCHMARK}
The real performance assessment of GNNs is not easy because the results reported in the paper may be closely related to the way the models are
implemented and trained and their hyper-parameters. Open Graph Benchmark(OGB)\cite{Hu2020OpenGB} is a diverse set of challenging and realistic benchmark datasets to facilitate scalable, robust, and reproducible graph machine learning (ML) research. It gives a representation of graph networks in various domains, such as biological networks, molecular graphs, source code ASTs, and knowledge graphs.

In addition to using PyTorch Geometric to implement models and evaluate them on OGB, Cogdl\cite{Cen2021CogDLAE} also gives a set of easy methods to implement graph neural networks, in which common datasets and GNN models are given. This work gives evaluation results for some of the popular GNN models, and users can easily reproduce the results in the leaderboard.


Graph Convolution Network (GCN)~\cite{kipf2016semi-GCN} propagates information from each node to its neighbors with a localized first-order approximation of spectral graph convolutions. Graph Attention Network (GAT)~\cite{Velickovic2018GraphAN} replaces the graph convolution layers with masked self-attentional layers, aiming to overcome the shortcomings of methods based on graph convolutions. PPNP and its fast approximation APPNP ~\cite{klicpera2019predict} also replace the power of graph convolution matrix with the PageRank matrix to solve the over-smoothing problem in GCN model. There are also extensions of GCN like GCNII~\cite{chen2020simple} which is a deeper graph neural network. GraphSAGE~\cite{Hamilton2017InductiveRL} is a general inductive framework that leverages node features information to generate node embeddings for previously unseen data.

